Global sensitivity analysis in Monte Carlo radiation transport

We consider Global Sensitivity Analysis for Monte Carlo radiation transport applications. GSA is usually combined with Uncertainty Quantification, where the latter quantifies the variability of a model output in the presence of uncertain inputs and the former attributes this variability to the inputs. The additional noise inherent to MC RT solvers due to the finite number of particle histories presents an additional challenge to GSA and UQ, which are well-established for deterministic solvers. In this contribution, we apply variance deconvolution to the Saltelli method to address MC RT solver noise without having to over-resolve the MC RT simulation.

==> sections/gsa_pce.tex <==
% The Polynomial Chaos (PC) method~\cite{Crestaux2009} is a popular choice in the UQ community.% to represent the response of a system by means of an orthogonal basis. 

Our companion paper~\cite{GeraciMC2023} introduces a PC strategy that we extend and adapt here to GSA.
%In this work, we rely on our %previous work~\cite{GeraciMC2021} and the 
%companion paper~\cite{GeraciMC2023} to extended and adapt the strategy proposed there to the GSA task.
% We note that the computation of GSA indices from PC is not a novel topic, however the formulation introduced in this work, which explicitly manages the MC RT stochasticity by embedding the variance deconvolution, has not been previously introduced. Here, we summarize the steps behind the computation of sensitivity indices, while we leave to the full manuscript the in-depth discussion of the algorithm. 
The PC surrogate is expressed a polynomial expansion which approximates the system's response as $Q^{PC}(\xi)$
\begin{equation}
 Q(\xi) \approx \sum_{k=0}^P \beta_k \Psi_k(\xi) = Q^{PC}(\xi),
\end{equation}
where $\Psi_k$ represents the $k^\text{th}$ term of a polynomial basis orthogonal to the PDF $p(\xi)$. %If a total polynomial degree $n_0$ is chosen (this could be determined adaptively, rater that decided beforehand, but we leave this angle to the full manuscript), the total number of terms is $P+1 = (n_0+d)! / (n_0! d!)$. 
As illustrated in~\cite{GeraciMC2023}, a non-intrusive spectral projection can be used to evaluate the coefficients as 
\begin{equation}
  \label{eq:NISP}
  \beta_k = \frac{ \EExi{ Q(\xi) \Psi_k(\xi) } }{ b_k }, \quad \mathrm{where} \quad b_k = \EExi{\Psi_k^2(\xi)},
\end{equation}
% The normalization coefficient $b_k$ can be obtained in closed form so it is a constant, \textit{i.e.} non-random, value. In the MC RT context, we need to consider the presence of both the stochasticity introduced by $\eta$ in addition to the uncertain parameters $\xi$, which allows to 
% express the coefficients as
% 
% In the radiation transport context, we are 
% interested in problems in which the system's response is itself a random variable obtained by solving transport quantities using a Monte Carlo (MC) solver. If we consider an elementary event $f$,
% \textit{i.e.} a MC particle history, a transport solution depends not only on the random vector $\xi$, but also on the intrinsic stochastic variables of the solvers. We denote this
% vector as $\eta$. In this case, the system response $Q$ is indeed obtained as a statistic of $f$ for each realization of $\xi$: we consider here $Q(\xi) = \EEeta{ f }$. By substituting the expression of the QoI $Q$ within Eq.~\ref{eq:NISP} we obtain 
% %the final expression of the $k$th PC coefficient for a problem based on stochastic solver described by the vector $\eta$
% \begin{equation}
%  \beta_k = \frac{1}{b_k} \EExi{ Q(\xi) \Psi_k(\xi) } = \frac{1}{b_k} \EExi{ \EEeta{f(\xi,\eta)} \Psi_k(\xi) } = \frac{1}{b_k} { \EE{f(\xi,\eta) \Psi_k(\xi)} },
% \end{equation} 
% which illustrates the need for sampling both $\xi$ and $\eta$. The standard way to proceed in a similar situation is to obtain very accurate MC solutions for each realization of $Q(\xi^{(i)})$ by using a large number of histories $N_\eta$ and subsequently integrate over $\xi$. However, an alternative approach consists in approximating directly
% the integral $\EE{f(\xi,\eta) \Psi_k(\xi)}$ by obtaining $N_{real}$ realizations in the combined space $(\xi,\eta)$. The two approaches correspond to 
% % is to sample directly in the combined $(\xi,\eta)$ space and approximate directly the 
% % combined integration with $N_{real}$ samples. We refer to the former as a segregated approach and the latter as a direct approach, which correspond to
% \begin{equation}
%  \beta_k = 
%  \left\{
%  \begin{split}
%     \frac{1}{b_k} \EExi{ \EEeta{f(\xi,\eta)} \Psi_k(\xi) } 
%      &\approx \frac{1}{b_k} \frac{1}{N_\xi} \sum_{i=1}^{N_\xi} \left( \frac{\Psi_k(\xi^{(i)})}{N_\eta} \sum_{j=1}^{N_\eta} f(\xi^{(i)},\eta^{(j)}) \right) 
%      \triangleq \hat{\beta}^s_k \quad \mathrm{(Segregated)} \\
%     \frac{1}{b_k} \EE{ f(\xi,\eta) \Psi_k(\xi) } &\approx \frac{1}{b_k} \frac{1}{N_{real}} \sum_{r=1}^{N_{real}} \left( f(\xi^{(r)},\eta^{(r)}) \Psi_k(\xi^{(r)})  \right) 
%      \triangleq \hat{\beta}^d_k \quad \mathrm{(Direct)} \\
%  \end{split}
%  \right.
% \end{equation}
and in the MC RT context,
\begin{equation}
 \beta_k = \frac{1}{b_k} \EExi{ \EEeta{f(\xi,\eta)} \Psi_k(\xi) } 
     \approx \frac{1}{b_k} \frac{1}{N_\xi} \sum_{i=1}^{N_\xi} \left( \frac{\Psi_k(\xi^{(i)})}{N_\eta} \sum_{j=1}^{N_\eta} f(\xi^{(i)},\eta^{(j)}) \right) 
     \triangleq \hat{\beta}_{k,N_\eta}~.
\end{equation}

PC is a convenient approach because %moments, like the expected value and the variance, and 
the sensitivity index of $u$ can be obtained directly %as function of 
from the coefficients, using the sum of all contributions which involve the variable(s) $u$~\cite{Crestaux2009} (collected in the set $K_u$),
\begin{equation}\label{eq:pce-si}
 S_u = \frac{\sum_{k \in K_u} (\hat{\beta}_{k,N_\eta})^2 b_k}{\Vxi{Q}}.
\end{equation}
%which corresponds to the sum of all contributions including the variable(s) $u$.

% \red{Add expression for the sensitivity indices}.
% Both choices represent an unbiased estimator, however their variances are different. 
% % our goal here is to show that the direct approach has a computational advantage for the same computational cost. 
% By using the law of total variance in the form $\Var{ \cdot } = \Var{ \EEeta{ \cdot } } + \EE{ \mathbb{V}ar_{\eta}\left[ \cdot \right] }$, it is 
% possible to derive the variance of the estimators $\hat{\beta}^s_k$ and $\hat{\beta}^d_k$ as
% % \begin{equation}
% % %  \begin{split}
% %   \Var{ \hat{\beta}^d_k } = \frac{ \Var{ \Psi_k(\xi) Q(\xi) } + \EE{ \Psi_k^2(\xi) \sigma^2(\xi) } }{N} \quad \mathrm{and} \quad
% %   \Var{ \hat{\beta}^s_k } = \frac{ \frac{\Var{ \Psi_k(\xi) Q(\xi) } }{N_\eta} + \EE{  \Psi_k^2(\xi) \sigma^2(\xi) } }{ N },
% % %  \end{split}
% % \end{equation}
% \begin{equation}
% %  \begin{split}
%   \Var{ \hat{\beta}^d_k } = \frac{ \Var{ \Psi_k Q } + \EE{ \Psi_k^2 \sigma^2 } }{N} \quad \mathrm{and} \quad
%   \Var{ \hat{\beta}^s_k } = \frac{ N_\eta \Var{ \Psi_k Q }  + \EE{  \Psi_k^2 \sigma^2 } }{ N },
% %  \end{split}
% \end{equation}
% where we assured the same cost of the estimators by choosing $N = N_{reals} = N_\xi N_\eta$ and we indicated with $\sigma^2$ the variance of the elementary event $f$ 
% over $\eta$, \textit{i.e.}  $\sigma^2(\xi) \triangleq \mathbb{V}ar_{\eta}\left[ f(\xi,\eta) \right]$. The comparison of the two expressions shows that 
% $\Var{ \hat{\beta}^d_k }<\Var{ \hat{\beta}^s_k }$ which means that for the same computational cost the PC coefficients are recovered more sharply for the direct approach, that the segregated approach yields successively higher efficiency for smaller $N_\eta$, and that the segregated approach reduces to the direct approach when $N_\eta=1$. 
%Moreover, if we consider the first PC coefficient $\beta_0$, we can remove the effect of the noise introduced by unconverged MC statistics as 
%\begin{equation}
% \begin{split}
%  \Var{ \hat{\beta}^s_0 } &= %\frac{ N_\eta \Var{ Q(\xi) } + \EE{  \sigma^2(\xi) } }{ N } 
%                           \frac{ \Var{ Q } + \frac{ \EE{  \sigma^2 } }{N_\eta} } { N_\xi } 
%                           = \frac{ \Var{ \hat{Q} }}{ N_\xi } \quad \rightarrow \quad \Var{ Q }  =  \Var{ \hat{Q} } - \frac{ \EE{  \sigma^2 } }{N_\eta},
% \end{split}
%\end{equation}
%where $\hat{Q}(\xi) \approx \EEeta{ f(\xi,\eta) }$ is the system response that one can observe in a MC ray tracing experiment. This relationship has been verified numerically
%and the results will be presented in the final manuscript for the sake of compactness.

% \subsection{Effect of the MC noise in the PC coefficient}
% We now consider the first PC coefficient $\beta_0$ which corresponds to the mean value of the system's response. Its variance, in the case of the segregated approach can be
% written as (note that $\Psi_0 = 1$ for any basis):
% \begin{equation}
%  \begin{split}
%   \Var{ \hat{\beta}^s_0 } &= %\frac{ N_\eta \Var{ Q(\xi) } + \EE{  \sigma^2(\xi) } }{ N } 
%                            \frac{ \Var{ Q(\xi) } + \frac{ \EE{  \sigma^2(\xi) } }{N_\eta} } { N_\xi } 
%                            = \frac{ \Var{ \hat{Q}(\xi) }}{ N_\xi } \quad \rightarrow \quad \Var{ Q(\xi) }  =  \Var{ \hat{Q}(\xi) } - \frac{ \EE{  \sigma^2(\xi) } }{N_\eta}
%  \end{split}
% \end{equation}
% where $\hat{Q}(\xi) \approx \EEeta{ f(\xi,\eta) }$ is the system response that one can observe in a MC ray tracing experiment. This relationship has been verified numerically
% and the results will be presented in the final manuscript.
% From this relationship, it is clear that one can 
% obtain the variance of the true system response $\Var{Q}$ by eliminating the noise contribution as
% \begin{equation}
%  \Var{ Q(\xi) }  =  \Var{ \hat{Q}(\xi) } - \frac{ \EE{  \sigma^2(\xi) } }{N_\eta}.
% \end{equation}


